Unsupervised Hyperbolic Representation Learning via Message Passing Auto-Encoders

Most of the existing literature regarding hyperbolic embedding concentrate upon supervised learning, whereas the use of unsupervised hyperbolic embedding is less well explored. In this paper, we analyze how unsupervised tasks can benefit from learned representations in hyperbolic space. To explore how well the hierarchical structure of unlabeled data can be represented in hyperbolic spaces, we design a novel hyperbolic message passing auto-encoder whose overall auto-encoding is performed in hyperbolic space. The proposed model conducts auto-encoding the networks via fully utilizing hyperbolic geometry in message passing. Through extensive quantitative and qualitative analyses, we validate the properties and benefits of the unsupervised hyperbolic representations. Codes are available at https://github.com/junhocho/HGCAE.

==> table_ablation_ic.tex <==
\begin{table}[t]
\caption{Ablation studies on image clustering.}
\vspace{-7mm}
\label{sample-table}
\begin{center}
\scriptsize
\begin{tabularx}{0.45\textwidth}{lYYYYYY}
\midrule
\multirow{2}{*}{} & \multicolumn{3}{c}{ImageNet-10} & \multicolumn{3}{c}{ImageNet-Dogs} \\
\cmidrule{2-7}
 & ACC & NMI & ARI & ACC & NMI & ARI \\
\midrule
CAE                   & 0.253 & 0.134 & 0.068 & 0.134 & 0.059 & 0.022 \\
CAE + HNN             & 0.298 & 0.155 & 0.093 & 0.142 & 0.068 & 0.029 \\
CAE + GAE             & 0.480 & 0.292 & 0.176 & 0.204 & 0.093 & 0.047 \\
\midrule
CAE + HGCAE-P         & 0.617 & 0.397 & 0.350 & 0.251 & 0.132 & 0.077 \\
\midrule
\end{tabularx}
\label{ablation4}
\end{center}
\vspace{-5mm}
\end{table}


==> table_classification.tex <==
\begin{table}[t]
\caption{Top-1 error on ImageNet-10 and new data.}
\vspace{-7mm}
\begin{center}
\scriptsize
\begin{tabularx}{0.45\textwidth}{lYYYY}
\midrule
\multirow{3}{*}{} & \multicolumn{2}{c}{ImageNet-10} & \multicolumn{2}{c}{New data} \\
\cmidrule{2-5}
& Top-1 & Top-5 & Top-1 & Top-5  \\
\midrule        
100\% data                                     & 0.542 & 0.540 & 0.565 & 0.564  \\
100\% data + focal loss \cite{lin2017focal}    & 0.590 & 0.555 & 0.598 & 0.567  \\
100\% data + Random 50\%                       & 0.688 & 0.712 & 0.673 & 0.640  \\
100\% data + Ambiguous 50\%                    & 0.688 & 0.712 & 0.673 & 0.640  \\
100\% data + Certain 50\%                      & 0.688 & 0.712 & 0.673 & 0.640  \\
\midrule
\end{tabularx}
\label{classification}
\end{center}
\vspace{-5mm}
\end{table}
